The exponential logic of sequentialization

Linear logic has provided new perspectives on proof-theory, denotational semantics and the study of programming languages. One of its main successes are proof-nets, canonical representations of proofs that lie at the intersection between logic and graph theory. In the case of the minimalist proof-system of multiplicative linear logic without units (MLL), these two aspects are completely fused: proof-nets for this system are graphs satisfying a correctness criterion that can be fully expressed in the language of graphs. For more expressive logical systems (containing logical constants, quantifiers and exponential modalities), this is not completely the case. The purely graphical approach of proof-nets deprives them of any sequential structure that is crucial to represent the order in which arguments are presented, which is necessary for these extensions. Rebuilding this order of presentation - sequentializing the graph - is thus a requirement for a graph to be logical. Presentations and study of the artifacts ensuring that sequentialization can be done, such as boxes or jumps, are an integral part of researches on linear logic. Jumps, extensively studied by Faggian and di Giamberardino, can express intermediate degrees of sequentialization between a sequent calculus proof and a fully desequentialized proof-net. We propose to analyze the logical strength of jumps by internalizing them in an extention of MLL where axioms on a specific formula, the jumping formula, introduce constrains on the possible sequentializations. The jumping formula needs to be treated non-linearly, which we do either axiomatically, or by embedding it in a very controlled fragment of multiplicative-exponential linear logic, uncovering the exponential logic of sequentialization.

==> multiple.tex <==
\begin{definition}
Given two formula occurrences $F$ and $F'$ in $R$,
  a jump from $F$ to $F'$ is then encoded in $R_J$ by grafting the following gadget
in the $!?\J$-box of $F$:  
 \vspace{\beforepn}
\begin{proofnet}
  \pnformulae{
    \pnf[jb]{$J$}~~~~\pnf[j]{$\J^\bot$}\\
  }
  \pnaxiom[ax]{jb,j}
  \pnbox{ax,jb,j}
  \pnprom{j}[!j]{$\oc \J^\bot$}
  \pnexp{}{jb}[?jb]{$\wn \J$}
  \pnexp{}{!j}[?!j]{$\wn \oc \J^\bot$}
\end{proofnet}
 connecting its left edge to the contraction link
  inside the box and pulling its right edge out of the box 
  up to the $?!\J^\bot$-contraction link of $F'$.  
\end{definition}
%
%Jumps from $F$ will be placed inside the $!?J$-box, jumps to $F$ will be plugged on 
%the contraction link $?!J^\bot$. More precisely:
%\begin{definition}
%  Given a proof-structure $R$ and two formula occurrences $F$ and $F'$ in $R$,
%  a jump from $F$ to $F'$ is encoded in $R_J$ by grafting the following gadget
%
% \vspace{\beforepn}
%\begin{proofnet}
%  \pnformulae{
%    \pnf[jb]{$J$}~~~~\pnf[j]{$J^\bot$}\\
%  }
%  \pnaxiom[ax]{jb,j}
%  \pnbox{ax,jb,j}
%  \pnprom{j}[!j]{$\oc J^\bot$}
%  \pnexp{}{jb}[?jb]{$\wn J$}
%  \pnexp{}{!j}[?!j]{$\wn \oc J^\bot$}
%\end{proofnet}
%
%
%  in the $!?J$-box of $F$, connecting its left edge to the contraction link
%  inside the box and pulling its right edge out of the box 
%  up to the $?!J^\bot$ contraction link of $F'$.  
%\end{definition}
The erasure operation defined on formulae and proofs is still defined with
our new rules.
 
\begin{definition}
Let $\pi$ be a $\MLL$ proof and $\L$ be a set of pairs of formula occurrences
such that if $(F,F') \in \L$ then $F\prec F'$. 
For every formula occurrences $F$ of $\pi$
%, let $k$ be the number of times
%$F$ appears on the left of a pair in $\L$ ($k = |\pi_1(\L)\cap \{F\}|$),
we define $\pi_J^F$ \emph{the jumps of $F$} to be the $\MLLJ$-proof:
\[\pi_J^F \qquad = \qquad \begin{prooftree}
    \infer0[wk$_0$]{\vdash \wn \J}
    \infer0[wk$_0$]{\vdash \wn\oc \J^\perp}
    \infer0[Ax]{\vdash \J,\J^\perp}
    \infer1[p]{\vdash \wn \J,\J^\perp}
    \infer1[$\oc$]{\vdash \wn \J, \oc \J^\perp}
    \delims{\left(}{\right)^{(F,\ \_)\in \L}}%{0\leq i \leq k}}
    \infer[double]3[mix]{\vdash \wn \J, \wn\oc\J^\perp, 
    \left(\wn \J, \oc \J^\perp\right)_{(F,\ \_)\in \L}}
    \infer[double]1[ctr]{\vdash \wn \J, \wn\oc\J^\perp,
    \left(\oc \J^\perp\right)_{(F,\ \_)\in \L}}
    \infer[double]1[p]{\vdash \wn \J, \wn\oc\J^\perp, 
    \left(\wn \oc \J^\perp\right)_{(F,\ \_)\in \L}}
    \infer1[$\oc$]{\vdash \oc \wn \J, \wn\oc\J^\perp, 
    \left(\wn \oc \J^\perp\right)_{(F,-)\in \L}}
\end{prooftree}
\]
We note $\theta_F$ for the set of $\wn\oc\J^\perp$ formulas in the conclusion.
\end{definition}

\begin{definition}
Let $\pi$ be a $\MLL$ proof and $\L$ be a set of pairs of formula occurrences
such that if $(F,F') \in \L$ then $F\prec F'$. 
We define $\pi_\L$ the \emph{proof $\pi$ with explicit jumps $\L$}
as the $\MLL_J$ proof defined by introducing the jumps associate to a formula 
occurrence via a tensor after its creation and connecting those jumps to their
targets via a parr just before they are used.

More formally, we proceed by induction on the structure of $\pi$:
\begin{itemize}
  \item If $\pi \ = \ $
    $\begin{prooftree}
        \infer0[Ax]{\vdash A, A^{\bot}}
  \end{prooftree}
  $ \quad it is replaced by \quad  $
  %\qquad \mapsto \qquad
  \begin{prooftree}
        \infer0[Ax]{\vdash A, A^{\bot}}
        \hypo{\pi_J^A}
        \infer2[$\otimes$]{\vdash A\otimes \oc\wn\J, A^\perp, \theta_A}
        \hypo{\pi_J^{A^\perp}}
        \infer2[$\otimes$]{\vdash A\otimes \oc\wn\J, A^\perp \otimes \oc\wn\J, \theta_A, \theta_{A^\perp}}
  \end{prooftree}
 $

 We can check that there is a one-to-one correspondence between $\wn\oc\J^\perp$ 
 formulas in the conclusion and pairs $(F,F')$ such that $F$ is in $\pi$
 and $F'$ has not been used yet and $(F,F') \in \L$ or $F=F'$,

  \item Otherwise,
let $r$ be the last rule of $\pi$ and let $F_1$, $F_2$ be the formulae
used by $r$. For every $F_i$, let $\pi'$ be the premise that contains it and 
let $\L'$ be the restriction of $\L$ to formula occurrences in $\pi'$, 
then  $\pi'_{J\L_i}$ is inductively defined and its environment contains 
one $\wn\oc\J^\perp$ formula for every pair $(F',F_i)\in \L$ plus one
extra. We connect them to $F_i$ via :
\[
  \begin{prooftree}
    \hypo{\pi'_{J\L_i}}
  \infer1[]{\vdash \Gamma, F_i, \wn\oc\J^\perp, 
  \left(\wn \oc \J^\perp\right)_{(F',F_i) \in \L}}
    \infer[double]1[ctr]{\vdash \Gamma, F_i, \wn\oc\J^\perp}
    \infer1[$\parr$]{\vdash \Gamma,F_i\parr \wn\oc\J^\perp}
  \end{prooftree}
\]

We then apply the rule $r$. 

If $r$ is not the cut rule then it creates
a new formula occurrence 
$(F_1\parr \wn\oc\J^\perp) \boxempty (F_2\parr \wn\oc\J^\perp)$.
As for the axiom rule, we introduce its jumps using a tensor:
\[
  \begin{prooftree}
    \hypo{\ldots}
    \infer1[r]{\vdash \Delta, (F_1\parr \wn\oc\J^\perp) \boxempty (F_2\parr \wn\oc\J^\perp)}
    \hypo{\qquad \quad \pi_J^{F_1\boxempty F_2}}
\infer2[$\otimes$]{\vdash \Delta,
\left((F_1\parr \wn\oc\J^\perp) \boxempty (F_2\parr \wn\oc\J^\perp)\right)
\otimes \oc \wn \J,
\wn\oc\J^\perp, \theta_{F_1\boxempty F_2}}
  \end{prooftree}
\]
Again, we can check that there is a one-to-one correspondence between $\wn\oc\J^\perp$ 
 formulas in the conclusion and pairs $(F,F')$ such that $F$ is in $\pi$
 and $F'$ has not been used yet and $(F,F') \in \L$ or $F=F'$.
\end{itemize}
\end{definition}

%\[
% \quad
%  \begin{prooftree}
%  \hypo{\vdash \Gamma, F, G}
%  \infer1[\(\parr\)]{\vdash \Gamma, F\parr G}
%  \end{prooftree}
%  \quad
%  \begin{prooftree}
%  \hypo{\vdash \Gamma, F}
%  \hypo{\vdash \Delta, G}
%  \infer2[\(\otimes\)]{\vdash \Gamma, \Delta, F\otimes G}
%  \end{prooftree}
%  \quad
%  \begin{prooftree}
%  \hypo{\vdash \Gamma, F}
%  \hypo{\vdash \Delta, F^\perp}
%  \infer2[cut]{\vdash \Gamma, \Delta}
%  \end{prooftree}
% \] 
%

\begin{proposition}
For $\pi$ a $\MLL$ proof and $\L$ a set of pairs of formula occurrences
such that if $(F,F') \in \L$ then $F\prec F'$, then
  $$\erasurej{\pi_{J\L}} = \pi$$
\end{proposition}
\begin{proof}
  Immediate, by induction on $\pi$.
\end{proof}

\begin{proposition}
  Let $R$ be a $\MLL$-proof-net, let $\pi$ be a sequentialization of $R$
  and let $\L$ be a set of pairs of formula occurrences of $\pi$ such that
  $\L \subseteq \prec_\pi$, then $R_{J\L}$ is a desequentialization of $\pi_{J\L}$ 
  and thus is a $\MLLJ$-proof net.
\end{proposition}
\begin{proof}
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

